Probes for Nearby Galaxies

Data are given for 16 extragalactic objects (predominantly AGN) behind the Magellanic Clouds and for 146 quasar candidates behind the nearby galaxies NGC 45, 185, 253, 2366, 2403 and 6822, IC 1613, M31 and M33. The Magellanic Cloud objects were identified by their X-ray emission, and precise optical and X-ray positions and optical photometry and spectra are presented for all of these. The quasar candidates surrounding the other nearby galaxies were identified through a CFHT slitless spectral survey. Although redshifts for only eight of these candidates have been obtained, previous observations indicate that the majority are likely to be quasars. A subsample of 49 of the brighter objects could confidently be used, in addition to the Magellanic Cloud sources, as probes of the gas in nearby galaxies for rotation curve studies, for studies of their halos, for comparison with higher redshift QSO absorption lines, or as references for proper motion studies.

==> crampton.tab1.tex <==
%\magnification\magstep1
\def\ub{\underbar}
\nopagenumbers
\noindent
T{\sevenrm{ABLE}} 1. X-ray Galaxies and AGN Behind the Magellanic Clouds
\vskip 5pt

\settabs 12\columns
\hrule
\vskip 2pt
\hrule
\vskip 5pt
\+ X-ray Source$^a$  && X-ray Position (J2000.0) 
&&& ~~ X-ray Count &&~ $V$ &Redshift & ~Finding & ~~Notes \cr
\+~~~ RX J &&~~~ R.A. &~~~~~~~~~~ Dec. && Rate$^b$ (cts s$^{-1}$)  &&&&
~Chart$^c$ \cr 
\vskip 5pt
\hrule
\vskip 5pt
\+0005.3$-$7427  && 00$^h$05$^m$19.5$^s$ 
& ~~~~~ $-$74$^{\circ}$26$^{\prime}$42$^{\prime\prime}$ 
&&0.0315 $\pm$0.0058 && 16.3 & 0.1316 
& ~~~$\times$  & ~~resolved galaxy \cr
\+~~~~= SMC 1 \cr
\vskip 2pt
\+0033.3$-$6915 && 00~~33~~21.5 & ~~~~~ $-$69~15~13 && 0.020 $\pm$0.003
 && 15.5 & 0.0975 & ~~~$\times$ & ~~cluster A2789; ~1.  \cr 
\+~~~~= SMC 70 \cr
\vskip 2pt
\+0119.5$-$7301 &&  01~~19~~30.3 & ~~~~~ $-$73~01~28 && 0.006 $\pm$0.002
&& 15.8 & 0.0656 & ~~~$\times$ & ~~cluster; ~2. \cr 
\+~~~~= SMC 66 \cr
\vskip 2pt
\+0135.4$-$7048 && 01~~35~~23.5 & ~~~~~ $-$70~48~29 && 0.010 $\pm$0.005 && 
17.9 & 0.0647 & ~~~$\times$ & ~~cluster?; ~3.  \cr 
\vskip 2pt
\+0136.4$-$7105 && 01~~36~~25.6 & ~~~~~ $-$71~05~25 && 0.0078 $\pm$0.0020 &&
 19.1 & 0.4598 & ~~~$\times$ &  \cr
\+~~~~= SMC 68 \cr
\vskip 2pt
\+0454.2$-$6643 && 04~~54~~10.6 & ~~~~~ $-$66~43~17 && 0.0082 $\pm$0.0023 &&
18.2 & 0.2279 & ~~~$\times$ &   \cr
\vskip 2pt
\+0503.1$-$6634   && 05~~03~~05.1 & ~~~~~ $-$66~33~47 && 0.0511 $\pm$0.0077 
&& 16.8 & 0.064 & ~~P1 &  \cr
\+~~~~= CAL F \cr 
\vskip 2pt
\+0517.3$-$7044  && 05~~17~~17.1 & ~~~~~ $-$70~44~03 && 0.0063 $\pm$0.0011 
&& 18.2 & 0.1688 & ~~P2 &  \cr
\+~~~~= CAL 21 \cr 
\vskip 2pt
\+0524.0$-$7011  && 05~~24~~02.4 & ~~~~~ $-$70~11~06 && 0.0338 $\pm$0.0052
 && 17.7 & 0.151 & ~~P1 & \cr
\+~~~~= CAL 32 \cr 
\vskip 2pt
\+0531.5$-$7130  && 05~~31~~32.5 & ~~~~~ $-$71~29~48 && 0.0140 $\pm$0.0040
 && 19.2 & 0.2214 & ~~P1 & ~~ \cr 
\+~~~~= CAL 46 \cr
\vskip 2pt
\+0532.0$-$6920 && 05~~31~~59.2 & ~~~~~ $-$69~19~52 &&0.0050 $\pm$0.0011 
&& 18.9 &  0.1495 & ~~P1 &  \cr 
\vskip 2pt
\+0534.0$-$7145 && 05~~34~~00.5 & ~~~~~ $-$71~45~28 && 0.0124 $\pm$0.0018 &&
 13.8 & 0.0242 & ~~~$\times$ & ~~large galaxy; ~4. \cr 
\vskip 2pt
\+0534.8$-$6739 && 05~~34~~45.7 & ~~~~~ $-$67~38~57 && 0.0045 $\pm$0.0011 
&& 17.8 & 0.0720 & ~~P2 & ~~`star' 2; ~5. \cr
\vskip 2pt
\+0547.8$-$6745 && 05~~47~~45.4 & ~~~~~ $-$67~45~03 && 0.0097 $\pm$0.0021 && 
20.5 & 0.3905 & ~~P2 & ~~radio source; ~6. \cr 
\vskip 2pt
\+0550.5$-$7110 && 05~~50~~32.1 & ~~~~~ $-$71~09~56 && 0.0024 $\pm$0.0007 &&
 19.9 & 0.4429 & ~~~$\times$ & ~~ \cr
\vskip 2pt
\+0550.6$-$6637 && 05~~50~~33.3 & ~~~~~ $-$66~36~59  && - - - - - - 
&& 17.0 &0.076 & ~~pub. & ~~7.  \cr
\+~~~~= CAL 91 \cr
\vskip 5pt
\hrule
\vskip 5pt
\noindent
\leftline{$^a$SMC sources: Wang \& Wu 1992; CAL sources, alternately
called LHG: Long et al.\ 1981} 
\leftline{$^bROSAT$-HRI count rate in 25$^{\prime\prime}$ diameter
aperture; unless otherwise specified, these are point sources }
\leftline{$^c$finding charts: ~$\times$: this paper; ~P1: ~Schmidtke et
al.\ 1994; ~P2: ~Cowley et al.\ 1997} 
\vskip 5pt
\leftline{\underbar{Notes:}}
\vskip 3pt
\leftline{1. extended X-ray source; count rate in 72$^{\prime\prime}$ 
cell; associated with a cluster of galaxies; $V$ mag measured }
\leftline{ ~~~~~~~~in 40$^{\prime\prime}$ aperture; z for central cD gal} 
\leftline{2.  extended X-ray source; count rate in  
72$^{\prime\prime}$ cell; optical galaxy $V$ mag measured in
28$^{\prime\prime}$ aperture;} 
\leftline{ ~~~~~~~~double nucleus (see text)} 
\leftline{3. extended X-ray source; count 
rate in 72$^{\prime\prime}$ cell; galaxy cluster?; z
for brightest galaxy within the X-ray contours} 
\leftline{4. X-ray point source in center of very large, optical
galaxy (Up 053448$-$7147.3, S0(r))} 
\leftline{ ~~~~~~~~ $V$ mag measured in 80$^{\prime\prime}$ aperture; 
spectrum has narrow [O II], [O III] emission} 
\leftline{5. ``note added in proof" in Paper 2 identifies this source with
`star' 2 } 
\leftline{6. compact radio source MDM 100 (Marx et al.\ 1997) } 
\leftline{7. {\it Einstein} count rate and finding chart (Cowley et al.\
1984); spectrum described (Cristiani et al.\ 1984)} 

\end



==> crampton.tab2.tex <==
%\magnification\magstep1
\def\ub{\underbar}
\nopagenumbers
\noindent
T{\sevenrm{ABLE}} 2. Grens Observations 
\vskip 5pt
\settabs 7\columns
\hrule
\vskip 2pt
\hrule
\vskip 5pt
\+ Galaxy & Plate No. & Exposure & Prism
&~~~~~~ 1950 Coordinates of Center \cr
\+ && ~ (min.) & Angle & ~~~~~~~~~ R.A. & ~~~~~~~~~~~~ Dec. \cr
\vskip 5pt
\hrule
\vskip 5pt
\+NGC 45  & ~~ 2482  & ~~~ 90 & ~~ 90$^{\circ}$ 
& ~~~~~  00$^h$11$^m$ 37$^s$  &~~~~~~~
$-$23$^{\circ}$37$^{\prime}$ 00$^{\prime\prime}$ \cr
\+M 31 - E $^a$ & ~~ 2481  & ~~~ 60 & ~~~~ 0 & ~~~~~  
00~~33~~58 &~~~~~~~ +40~~51~~14 \cr
\+M 31 - C29 & ~~ 2466  & ~~~ 60 & ~ 245 & ~~~~~ 00~~47~~53 &~~~~~~~
+39~~51~~51 \cr 
\+NGC 185 & ~~ 1499  & ~~~ 90 & ~~~~ 0 & ~~~~~ 00~~36~~13 &~~~~~~~ 
+48~~03~~49 \cr
\+NGC 253 & ~~ 2483  & ~~~ 90 & ~~ 90 & ~~~~~ 00~~45~~10 
&~~~~~~~ $-$25~~33~~39 \cr
\+IC 1613 & ~~ 2476  & ~~~ 90 & ~~ 90 & ~~~~~ 01~~02~~23 &~~~~~~~ 
+01~~51~~53 \cr
\+M 33 - A   & ~~ 1496  & ~~~ 75 & ~ 270 & ~~~~~ 01~~31~~11 &~~~~~~~ 
+30~~39~~11 \cr
\+        & ~~ 2477  & ~~~ 90 & ~ 180 &    \cr
\+M 33 - B   & ~~ 1501  & ~~~ 90 & ~ 270 & ~~~~~ 
01~~32~~47 &~~~~~~~ +30~~15~~10 \cr
\+        & ~~ 2484  & ~~~ 90 & ~ 180 &&  \cr
\+M 33 - C   & ~~ 1489  & ~~~ 55 & ~~~~ 0  
& ~~~~~ 01~~31~~05 &~~~~~~~ +30~~39~~11 \cr
\+        & ~~ 2471  & ~~~ 90 & ~ 270 &&   \cr
\+NGC 2366 & ~~ 2478 & ~~~ 90 & ~ 300 & ~~~~~ 07~~23~~42 &~~~~~~~ 
+69~~19~~05 \cr
\+NGC 2403 & ~~ 2485  & ~~~ 90 & ~ 300 & ~~~~~ 07~~32~~14 &~~~~~~~ 
+65~~42~~32 \cr
\+NGC 6822 & ~~ 1484  & ~~~ 60 & ~~~~ 0 & ~~~~~ 
19~~42~~10 &~~~~~~~ $-$14~~55~~56 \cr
\+         & ~~ 1498  & ~~~ 90 & ~ 190 &&   \cr
\+         & ~~ 2463  & ~~ 155 & ~ 157 && \cr
\+         & ~~ 2474  & ~~~ 90 & ~~ 90 &&   \cr
\vskip 5pt
\hrule
\vskip 5pt
\noindent
$^a$ Close to C12 (Sargent et al. 1977)
\end



==> crampton.tab3.tex <==
\def\ub{\underbar}
\nopagenumbers
\noindent
T{\sevenrm{ABLE}} 3. Quasar Candidates Around Nearby Galaxies

\vskip 5pt
\settabs 10\columns
\hrule
\vskip 2pt
\hrule
\vskip 5pt
\+~~ Quasar && I.D.  &~~~J2000 Coordinates  && ~~~~~~~~m$_J$ 
& ~ Class & Emission Lines$^a$ \& Comments$^b$ \cr 
\+ Candidates &&& && & & \cr
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{NGC 45 Quasars:}
\vskip 5pt 
\+0012.3$-$2305 && 15  & $00^h12^m19\rlap{.}^s0$
&~~~$-23^{\circ}05^{\prime}33^{\prime \prime}$ &~~~~~~ 21.0 & ~~~~4 &
5200; red; high z?  \cr 
\+0012.3$-$2331 && 31  & 00 ~12 ~23.7 & ~~~$-$23 31 29 &~~~~~~ 20.8 &
~~~~4 &poor focus; W of pair  \cr 
\+0012.8$-$2308 && F   & 00 ~12 ~51.5 & ~~~$-$23 08 13 &~~~~~~ 19.9 &
~~~~2 &4320,3400; z = 1.8 \cr 
\+0013.2$-$2302 && C   & 00 ~13 ~13.3 & ~~~$-$23 02 46 &~~~~~~ 17.5 &
~~~~5 &dA \cr 
\+0013.4$-$2324 && 25  & 00 ~13 ~25.6 & ~~~$-$23 24 40 &~~~~~~ 21.0 &
~~~~4 &emission? short spectrum  \cr 
\+0013.4$-$2304 && G   & 00 ~13 ~27.5 & ~~~$-$23 04 45 &~~~~~~ 21.0 &
~~~~2 &4100,5200 \cr 
\+0013.5$-$2332 && N   & 00 ~13 ~35.2 & ~~~$-$23 32 32 &~~~~~~ 20.0 &
~~~~2 &4120  \cr 
\+0013.7$-$2306 && H   & 00 ~13 ~44.0 & ~~~$-$23 06 18 &~~~~~~ 19.1 &
~~~~2 &4200,5100 \cr 
\+0013.7$-$2259 && D   & 00 ~13 ~46.5 & ~~~$-$22 59 39 &~~~~~~ 21.3 &
~~~~1 &3840,4900; z = 2.2   \cr 
\+0013.8$-$2328 && O   & 00 ~13 ~51.4 & ~~~$-$23 28 34 &~~~~~~ 21.1 &
~~~~4 & \cr 
\+0013.9$-$2319 && M   & 00 ~13 ~54.2 & ~~~$-$23 19 32 &~~~~~~ 21.2 &
~~~~4 & \cr 
\+0013.9$-$2316 && J   & 00 ~13 ~56.2 & ~~~$-$23 16 00 &~~~~~~ 21.0 &
~~~~3 &3875 \cr 
\+0013.9$-$2327 && P   & 00 ~13 ~58.5 & ~~~$-$23 27 00 &~~~~~~ 20.8 &
~~~~4 &3980 \cr 
\+0014.0$-$2250 && B   & 00 ~14 ~00.4 & ~~~$-$22 50 17 &~~~~~~ 19.7 &
~~~~4 \cr 
\+0014.1$-$2309 && 12  & 00 ~14 ~08.8 & ~~~$-$23 09 35 &~~~~~~ 18.5 &
~~~~4 &blue object; emission from NGC 45?  \cr 
\+0014.2$-$2328 && 28  & 00 ~14 ~13.2 & ~~~$-$23 28 34 &~~~~~~ 20.4 &
~~~~4 &overlap; W of pair \cr 
\+0014.4$-$2259 && E   & 00 ~14 ~29.2 & ~~~$-$22 59 02 &~~~~~~ 21.2 &
~~~~1 &3840,4890; z = 2.2 \cr 
\+0014.5$-$2303 && 8   & 00 ~14 ~31.4 & ~~~$-$23 03 18 &~~~~~~ 21.1 &
~~~~4 & \cr 
\+0014.7$-$2303 && I   & 00 ~14 ~44.6 & ~~~$-$23 03 12 &~~~~~~ 20.0 &
~~~~3 &3750  \cr 
\+0014.8$-$2317 && S   & 00 ~14 ~50.6 & ~~~$-$23 17 49 &~~~~~~ 21.4 &
~~~~4 \cr 
\+0014.9$-$2309 && K   & 00 ~14 ~56.2 & ~~~$-$23 09 36 &~~~~~~ 20.2 &
~~~~4 &4100  \cr 
\+0014.9$-$2327 && V   & 00 ~14 ~57.5 & ~~~$-$23 27 39 &~~~~~~ 20.0 &
~~~~3 &3400,3850,4300; z = 1.8 \cr 
\+0014.4$-$2321 && R   & 00 ~14 ~26.7 & ~~~$-$23 21 19 &~~~~~~ 20.9 &
~~~~4 &3600  \cr 
\+0015.0$-$2320 && U   & 00 ~15 ~04.2 & ~~~$-$23 20 37 &~~~~~~ 20.2 &
~~~~4 &4060 \cr 
\+0015.2$-$2312 && T   & 00 ~15 ~14.7 & ~~~$-$23 12 37 &~~~~~~ 18.4 &
~~~~3 &4500,3900,5200  \cr 
\+0015.3$-$2306 && L   & 00 ~15 ~23.4 & ~~~$-$23 06 30 &~~~~~~ 21.2 &
~~~~4 &\cr 
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{M 31 -- Field E Quasars:}
\vskip 5pt
\+0035.3+4107 && F   & 00$^h$35$^m$18$\rlap{.}^s$8 &
~~~$+41^{\circ}07^{\prime}02^{\prime\prime}$ &~~~~~~ 16.5 & ~~~~5 & \cr 
\+0035.7+4046 && A   & 00 ~35 ~46.2 & ~~~+40 46 19 &~~~~~~ 18.9 & ~~~~2
&4960,4025; z = 1.6?  \cr 
\+0035.7+4134 && 5   & 00 ~35 ~46.6 & ~~~+41 34 02 &~~~~~~ 18.5 & ~~~~3 &
\cr 
\+0035.8+4053 && C   & 00 ~35 ~49.7 & ~~~+40 53 57 &~~~~~~ 16.9 & ~~~~5 & 
\cr 
\+0035.9+4056 && E   & 00 ~35 ~54.4 & ~~~+40 56 17 &~~~~~~ 20.9 & ~~~~3
&3920,5210  \cr 
\+0035.9+4112 && K   & 00 ~35 ~57.8 & ~~~+41 12 21 &~~~~~~ 20.3 & ~~~~2
&3550 \cr 
\+0036.3+4117 && O   & 00 ~36 ~19.2 & ~~~+41 17 48 &~~~~~~ 20.0 & ~~~~3
&4000 \cr 
\+0036.4+4125 && T   & 00 ~36 ~24.9 & ~~~+41 25 37 &~~~~~~ 21.1 & ~~~~4
&4140 \cr 
\+0036.4+4130 && U   & 00 ~36 ~26.7 & ~~~+41 30 09 &~~~~~~ 17.8 & ~~~~5
&dA \cr 
\+0036.4+4105 && J   & 00 ~36 ~29.6 & ~~~+41 05 02 &~~~~~~ 20.2 & ~~~~1
&4120,5170; z = 2.4  \cr 
\+0036.6+4134 && 8   & 00 ~36 ~40.1 & ~~~+41 34 35 &~~~~~~ 20.7 & ~~~~4
&4500  \cr 
\+0036.9+4120 && S   & 00 ~36 ~55.1 & ~~~+41 20 25 &~~~~~~ 20.5 & ~~~~4
&4800,4100  \cr 
\+0036.9+4101 && I   & 00 ~36 ~54.1 & ~~~+41 01 57 &~~~~~~ 20.6 & ~~~~4
&4140 \cr 
\+0036.9+4119 && R   & 00 ~36 ~59.2 & ~~~+41 19 25 &~~~~~~ 20.5 & ~~~~1
&4760,3960 \cr 
\+0037.6+4053 && H   & 00 ~37 ~41.5 & ~~~+40 53 47 &~~~~~~ 20.5 & ~~~~4 & 
\cr 
\+0037.6+4049 && G   & 00 ~37 ~41.5 & ~~~+40 49 55 &~~~~~~ 20.5 & ~~~~3
&3780,4200  \cr 
\+0037.8+4103 && M   & 00 ~37 ~53.4 & ~~~+41 03 00 &~~~~~~ 20.3 & ~~~~4
&4000 \cr 
\+0037.9+4104 && N   & 00 ~37 ~56.7 & ~~~+41 04 54 &~~~~~~ 20.3 & ~~~~4
&3840 \cr 
\+0038.4+4106 && Q   & 00 ~38 ~27.0 & ~~~+41 06 50 &~~~~~~ 17.2 & ~~~~5
&dA \cr 
\vskip 3pt
\hrule
\vfill\eject
\noindent
T{\sevenrm{ABLE}} 3. (continued)
\vskip 8pt
\hrule
\vskip 2pt
\hrule
\vskip 5pt
\+~~ Quasar && I.D.  &~~~J2000 Coordinates  && ~~~~~~~~m$_J$ 
& ~ Class & Emission Lines$^a$ \& Comments$^b$ \cr 
\+ Candidates &&& && & & \cr
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{M 31 -- Field C29 Quasars:}
\vskip 5pt
\+0048.8+4009 && O   & 00$^h48^m52\rlap{.}^s7$ &
~~~$+40^{\circ}09^{\prime}18^{\prime\prime}$ &~~~~~~ 17.9 & ~~~~4 & 4040
\cr 
\+0048.9+4005 && V   & 00 ~48 ~58.4 & ~~~+40 05 13 &~~~~~~ 18.5 & ~~~~4
&white dwarf? \cr 
\+0049.5+4006 && U   & 00 ~49 ~33.2 & ~~~+40 06 13 &~~~~~~ 18.9 & ~~~~2
&3750,4630; z = 1.4  \cr 
\+0049.6+3952 && H   & 00 ~49 ~41.0 & ~~~+39 52 50 &~~~~~~ 20.4 & ~~~~2 &
4160 \cr 
\+0050.1+3958 && I   & 00 ~50 ~07.8 & ~~~+39 58 09 &~~~~~~ 19.4 & ~~~~3
&4000; very  weak line(s) \cr 
\+0050.2+3941 && P   & 00 ~50 ~13.7 & ~~~+39 41 24 &~~~~~~ 19.8 & ~~~~4
&4030,3540 \cr 
\+0050.3+4006 && L   & 00 ~50 ~20.4 & ~~~+40 06 22 &~~~~~~ 21.0 & ~~~~4
&4040; very weak lines  \cr 
\+0051.1+4017 && N   & 00 ~51 ~08.4 & ~~~+40 17 38 &~~~~~~ 20.5 & ~~~~4 &
\cr 
\+0051.2+3954 && F   & 00 ~51 ~14.7 & ~~~+39 54 55 &~~~~~~ 19.0 & ~~~~2
&4590,5160 \cr 
\+0051.3+3947 && C   & 00 ~51 ~21.1 & ~~~+39 47 13 &~~~~~~ 20.4 & ~~~~4
&5120,3950  \cr 
\+0051.4+3950 && D   & 00 ~51 ~25.2 & ~~~+39 50 06 &~~~~~~ 19.3 & ~~~~1
&4080,5160; z = 2.4  \cr 
\+0051.5+3955 && R   & 00 ~51 ~31.3 & ~~~+39 55 49 &~~~~~~ 20.4 & ~~~~4 &
\cr 
\+0051.8+3942 && 2   & 00 ~51 ~52.8 & ~~~+39 42 50 &~~~~~~ 18.1 & ~~~~4 &
\cr 
\+0052.1+3951 && Q   & 00 ~52 ~07.2 & ~~~+39 51 58 &~~~~~~ 20.6 & ~~~~4 &
\cr 
\+0052.2+4019 && 14  & 00 ~52 ~13.9 & ~~~+40 19 11 &~~~~~~ 20.9 & ~~~~4 &
\cr 
\+0052.2+4012 && J   & 00 ~52 ~15.7 & ~~~+40 12 52 &~~~~~~ 20.2 & ~~~~2 &
4530 \cr 
\+0052.3+3944 && B   & 00 ~52 ~23.3 & ~~~+39 44 40 &~~~~~~ 20.2 & ~~~~3
&4740,3950; z = 2.9? \cr 
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{NGC 185 Quasars:}
\vskip 5pt

\+0037.4+4803 && D   & 00$^h37^m27\rlap{.}^s5$ &
~~~$+48^{\circ}03^{\prime}29^{\prime\prime}$ &~~~~~~ 18.0 & ~~~~3
&3725,4925; white dwarf? \cr 
\+0039.6+4817 && H   & 00 ~39 ~40.7 & ~~~+48 17 58 &~~~~~~ 19.0 & ~~~~2
&3600,4600   \cr 
\+0039.8+4802 && G   & 00 ~39 ~48.4 & ~~~+48 02 57 &~~~~~~ 19.4 & ~~~~2
&3750  \cr 
\+0040.9+4820 && K   & 00 ~40 ~56.9 & ~~~+48 20 18 &~~~~~~ 19.7 & ~~~~4 &
\cr 
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{NGC 253 Quasars:}
\vskip 5pt
\+0045.7$-$2515 && H   & 00$^h45^m43\rlap{.}^s0$ &
~~~$-25^{\circ}15^{\prime}35^{\prime\prime}$ &~~~~~~ 19.9 & ~~~~4 &4980; ~* \cr 
\+0045.9$-$2503 && V   & 00 ~45 ~59.6 & ~~~$-$25 03 56 &~~~~~~ 21.2 &
~~~~3 &3880  \cr 
\+0046.1$-$2503 && W   & 00 ~46 ~11.8 & ~~~$-$25 03 32 &~~~~~~ 19.8 &
~~~~3 &5000  \cr 
\+0046.3$-$2528 && N   & 00 ~46 ~22.4 & ~~~$-$25 28 20 &~~~~~~ 20.9 &
~~~~1 &4550; z = 2.7? \cr 
\+0046.3$-$2532 && R   & 00 ~46 ~22.1 & ~~~$-$25 32 37 &~~~~~~ 20.8 &
~~~~4 &4060  \cr 
\+0046.5$-$2457 && U   & 00 ~46 ~32.6 & ~~~$-$24 57 20 &~~~~~~ 21.3 &
~~~~3 &5100  \cr 
\+0046.5$-$2518 && Y   & 00 ~46 ~30.9 & ~~~$-$25 18 15 &~~~~~~ 21.2 &
~~~~3 &3900 \cr 
\+0046.6$-$2529 && O   & 00 ~46 ~36.6 & ~~~$-$25 29 28 &~~~~~~ 19.9 &
~~~~3 &3460,5120  \cr 
\+0046.6$-$2508 && E   & 00 ~46 ~39.3 & ~~~$-$25 08 33 &~~~~~~ 21.0 &
~~~~1 &4140,4800,5220; z = 2.4 \cr 
\+0046.6$-$2500 && B   & 00 ~46 ~41.8 & ~~~$-$25 00 27 &~~~~~~ 20.0 &
~~~~3 &4300 \cr 
\+0046.7$-$2519 && I   & 00 ~46 ~43.6 & ~~~$-$25 19 34 &~~~~~~ 21.2 &
~~~~2 &4010 \cr 
\+0046.7$-$2521 && J   & 00 ~46 ~47.5 & ~~~$-$25 21 51 &~~~~~~ 20.9 &
~~~~4 &3830; brighter on grens plate  \cr 
\+0046.9$-$2531 && A2  & 00 ~46 ~55.6 & ~~~$-$25 31 22 &~~~~~~ 21.0 &
~~~~4 &5100?  \cr 
\+0048.1$-$2459 && C   & 00 ~48 ~08.7 & ~~~$-$24 59 11 &~~~~~~ 20.7 &
~~~~4 &3750   \cr 
\+0048.1$-$2535 && S   & 00 ~48 ~08.0 & ~~~$-$25 35 07 &~~~~~~ 19.8 &
~~~~1 &4330; ~* \cr 
\+0048.3$-$2523 && K   & 00 ~48 ~23.0 & ~~~$-$25 23 53 &~~~~~~ 20.8 &
~~~~4 &4100?; overlap?  \cr 
\+0048.3$-$2510 && F   & 00 ~48 ~23.2 & ~~~$-$25 10 10 &~~~~~~ 21.3 &
~~~~4 &4170  \cr 
\+0048.4$-$2528 && P   & 00 ~48 ~27.0 & ~~~$-$25 28 58 &~~~~~~ 18.8 &
~~~~3 &3920    \cr 
\+0048.7$-$2512 && X   & 00 ~48 ~44.7 & ~~~$-$25 12 06 &~~~~~~ 21.0 &
~~~~4 &4300 \cr 
\+0048.7$-$2529 && Q   & 00 ~48 ~44.1 & ~~~$-$25 29 40 &~~~~~~ 20.7 &
~~~~3 &3860  \cr 
\+0049.2$-$2525 && M   & 00 ~49 ~17.2 & ~~~$-$25 25 57 &~~~~~~ 19.6 &
~~~~4 & \cr 
\+0049.2$-$2524 && L   & 00 ~49 ~17.9 & ~~~$-$25 24 42 &~~~~~~ 20.6 &
~~~~3 &3800  \cr 
\vskip 3pt
\hrule
\vfill\eject
\noindent
T{\sevenrm{ABLE}} 3. (continued)
\vskip 5pt
\hrule
\vskip 2pt
\hrule
\vskip 5pt
\+~~ Quasar && I.D.  &~~~J2000 Coordinates  && ~~~~~~~~m$_J$ 
& ~ Class & Emission Lines$^a$ \& Comments$ba$ \cr 
\+ Candidates &&& && & & \cr
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{IC 1613 Quasars:}
\vskip 5pt
\+0102.9+0154 && V   & 01$^h02^m57\rlap{.}^s5$ &
~~~$+01^{\circ}54^{\prime}49^{\prime\prime}$ &~~~~~~ 19.4 & ~~~~4 & 4750
\cr 
\+0103.1+0202 && P   & 01 ~03 ~08.5 & ~~~+02 02 18 &~~~~~~ 18.3 & ~~~~2
&3530,4450; ~*  \cr 
\+0103.2+0204 && O   & 01 ~03 ~12.0 & ~~~+02 04 14 &~~~~~~ 20.2 & ~~~~2
&4420,5100  \cr 
\+0103.5+0150 && W   & 01 ~03 ~30.8 & ~~~+01 50 41 &~~~~~~ 19.1 & ~~~~4
&3700 \cr 
\+0103.6+0212 && J   & 01 ~03 ~36.9 & ~~~+02 12 32 &~~~~~~ 21.2 & ~~~~3
&4000 \cr 
\+0103.6+0212 && K   & 01 ~03 ~39.2 & ~~~+02 12 48 &~~~~~~ 21.2 & ~~~~3
&3900 \cr 
\+0103.8+0224 && B   & 01 ~03 ~52.5 & ~~~+02 24 00 &~~~~~~ 21.3 & ~~~~3
&~* \cr 
\+0104.1+0224 && C   & 01 ~04 ~06.9 & ~~~+02 24 57 &~~~~~~ 20.4 & ~~~~3
&4050 \cr 
\+0104.2+0209 && L   & 01 ~04 ~14.9 & ~~~+02 09 28 &~~~~~~ 21.1 & ~~~~4
&4000  \cr 
\+0104.3+0220 && I   & 01 ~04 ~20.0 & ~~~+02 20 11 &~~~~~~ 20.6 & ~~~~2
&4100,5050; z = 1.6  \cr 
\+0104.7+0222 && E   & 01 ~04 ~44.0 & ~~~+02 22 16 &~~~~~~ 21.3 & ~~~~2
&3900  \cr 
\+0104.7+0225 && D   & 01 ~04 ~47.7 & ~~~+02 25 02 &~~~~~~ 21.2 & ~~~~1
&4750,4020; z = 2.9 \cr 
\+0104.9+0152 && Y   & 01 ~04 ~59.6 & ~~~+01 52 20 &~~~~~~ 19.8 & ~~~~4
&3900 \cr 
\+0105.0+0201 && S   & 01 ~05 ~05.3 & ~~~+02 01 08 &~~~~~~ 21.3 & ~~~~4
& \cr 
\+0105.6+0158 && A2  & 01 ~05 ~40.0 & ~~~+01 58 14 &~~~~~~ 20.7 & ~~~~4 &
\cr 
\+0105.7+0211 && M   & 01 ~05 ~43.7 & ~~~+02 11 31 &~~~~~~ 21.5 & ~~~~4
&4100 \cr 
\+0105.7+0152 && E2  & 01 ~05 ~44.1 & ~~~+01 52 10 &~~~~~~ 21.4 & ~~~~4
&5050; z = 3.2? \cr 
\+0105.9+0214 && N   & 01 ~05 ~54.2 & ~~~+02 14 06 &~~~~~~ 21.0 & ~~~~4
&3760,4680  \cr 
\+0106.0+0200 && U   & 01 ~06 ~00.3 & ~~~+02 00 30 &~~~~~~ 21.0 & ~~~~3
&4670 \cr 
\+0106.0+0220 && G   & 01 ~06 ~01.1 & ~~~+02 20 53 &~~~~~~ 20.7 & ~~~~3
&3900  \cr 
\+0106.3+0220 && H   & 01 ~06 ~22.3 & ~~~+02 20 50 &~~~~~~ 20.3 & ~~~~3
&4030 \cr 
\+0106.4+0158 && C2  & 01 ~06 ~27.1 & ~~~+01 58 46 &~~~~~~ 21.3 & ~~~~4
&3625,4140  \cr 
\+0106.7+0211 && F2  & 01 ~06 ~42.3 & ~~~+02 11 27 &~~~~~~ 19.5 & ~~~~4
&3925? \cr 
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{M 33 Quasars:}
\vskip 5pt
\+0132.1+3022 && A89 & 01$^h32^m10\rlap{.}^s0$ &
~~~$+30^{\circ}22^{\prime}57^{\prime\prime}$ &~~~~~~ 16.7 & ~~~~5 & dA \cr
\+0132.6+3107 && J77 & 01 ~32 ~40.2 & ~~~+31 07 50 &~~~~~~ 18.7 & ~~~~4
&overlap?  \cr 
\+0134.0+3118 && I77 & 01 ~34 ~00.5 & ~~~+31 18 09 &~~~~~~ 19.8 & ~~~~1
&4025,5090; z = 2.3  \cr 
\+0134.6+3114 && C77 & 01 ~34 ~37.8 & ~~~+31 14 48 &~~~~~~ 20.1 & ~~~~2
&4150,5200   \cr 
\+0135.7+3035 && D84 & 01 ~35 ~43.6 & ~~~+30 35 35 &~~~~~~ 20.6 & ~~~~4
&4085  \cr 
\+0135.3+3027 && E84 & 01 ~35 ~23.1 & ~~~+30 27 26 &~~~~~~ 20.7 & ~~~~3
&3800?   \cr 
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{NGC 2366 Quasars:}
\vskip 5pt
\+0726.2+6909 && F   & 07$^h26^m17\rlap{.}^s8$ &
~~~$+69^{\circ}09^{\prime}22^{\prime\prime}$ &~~~~~~ 20.4 & ~~~~2
&3820,4800; z = 2.1  \cr 
\+0726.4+6856 && S   & 07 ~26 ~26.2 & ~~~+68 56 26 &~~~~~~ 20.4 & ~~~~4
&4080  \cr 
\+0726.5+6857 && P   & 07 ~26 ~30.8 & ~~~+68 57 51 &~~~~~~ 17.2 & ~~~~4
&~* \cr 
\+0729.3+6857 && D   & 07 ~29 ~21.3 & ~~~+68 57 45 &~~~~~~ 18.2 & ~~~~1
&3880  \cr 
\+0729.7+6901 && G   & 07 ~29 ~43.2 & ~~~+69 01 19 &~~~~~~ 20.4 & ~~~~2
&3750 \cr 
\+0729.7+6914 && X   & 07 ~29 ~44.4 & ~~~+69 14 19 &~~~~~~ 20.5 & ~~~~4
&3700 \cr 
\+0729.7+6855 && U   & 07 ~29 ~42.5 & ~~~+68 55 51 &~~~~~~ 19.4 & ~~~~5
& \cr 
\+0729.9+6904 && V   & 07 ~29 ~54.7 & ~~~+69 04 31 &~~~~~~ 21.1 & ~~~~3
&4100 \cr 
\+0730.6+6851 && B   & 07 ~30 ~38.9 & ~~~+68 51 51 &~~~~~~ 20.5 & ~~~~2
&4330,5000 \cr 
\+0730.9+6920 && L   & 07 ~30 ~59.3 & ~~~+69 20 21 &~~~~~~ 20.4 & ~~~~3
&3970 \cr 
\+0732.2+6905 && I   & 07 ~32 ~15.5 & ~~~+69 05 10 &~~~~~~ 20.6 & ~~~~3
&3600 \cr 
\+0732.8+6909 && W   & 07 ~32 ~50.7 & ~~~+69 09 33 &~~~~~~ 16.3 & ~~~~5
&dA white dwarf \cr 
\vskip 5pt
\hrule
\vfill\eject
\noindent
T{\sevenrm{ABLE}} 3. (concluded)
\vskip 5pt
\hrule
\vskip 2pt
\hrule
\vskip 5pt
\+~~ Quasar && I.D.  &~~~J2000 Coordinates  && ~~~~~~~~m$_J$ 
& ~ Class & Emission Lines$^a$ \& Comments$^b$ \cr 
\+ Candidates &&& && & & \cr
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{NGC 2403 Quasars:}
\vskip 5pt
\+0734.2+6548 && P   & 07$^h34^m13\rlap{.}^s8$ &
$~~~+65^{\circ}48^{\prime}49^{\prime\prime}$ &~~~~~~ 19.2 & ~~~~4 & 3920
\cr 
\+0734.6+6536 && I   & 07 ~34 ~37.9 & ~~~+65 36 17 &~~~~~~ 20.9 & ~~~~2
&4400  \cr 
\+0734.8+6555 && S   & 07 ~34 ~51.2 & ~~~+65 55 38 &~~~~~~ 19.2 & ~~~~3
&4150; ~* \cr 
\+0735.1+6548 && O   & 07 ~35 ~08.0 & ~~~+65 48 19 &~~~~~~ 19.2 & ~~~~2
&4100,3550; ~*  \cr 
\+0735.1+6553 && R   & 07 ~35 ~09.2 & ~~~+65 53 05 &~~~~~~ 19.4 & ~~~~3
&3500; ~* \cr 
\+0735.5+6535 && K   & 07 ~35 ~31.5 & ~~~+65 35 06 &~~~~~~ 20.3 & ~~~~4
&3850? \cr 
\+0735.7+6520 && E   & 07 ~35 ~45.2 & ~~~+65 20 36 &~~~~~~ 20.8 & ~~~~2
&5050 \cr 
\+0737.2+6557 && V   & 07 ~37 ~16.4 & ~~~+65 57 39 &~~~~~~ 20.3 & ~~~~4
&5200 \cr 
\+0737.5+6508 && D   & 07 ~37 ~35.6 & ~~~+65 08 25 &~~~~~~ 18.4 & ~~~~2
&3900,5000; ~*    \cr 
\+0737.8+6516 && F   & 07 ~37 ~52.5 & ~~~+65 16 36 &~~~~~~ 20.4 & ~~~~4
&4000,4950  \cr 
\+0738.3+6536 && N   & 07 ~38 ~23.7 & ~~~+65 36 40 &~~~~~~ 19.9 & ~~~~2
&4320; ~* \cr 
\+0739.2+6528 && M   & 07 ~39 ~13.8 & ~~~+65 28 11 &~~~~~~ 19.7 & ~~~~4
&3800 \cr 
\+0740.4+6534 && Q   & 07 ~40 ~24.0 & ~~~+65 34 19 &~~~~~~ 18.5 & ~~~~4
&~* \cr 
\+0740.4+6539 && U   & 07 ~40 ~24.7 & ~~~+65 39 57 &~~~~~~ 19.4 & ~~~~2
&4400; ~* \cr 
\vskip 3pt
\hrule
\vskip 5pt
\noindent
\ub{NGC 6822 Quasars:}
\vskip 5pt
\+1943.9$-$1502 && Q   & 19$^h43^m58\rlap{.}^s9$ &
~~~$-15^{\circ}02^{\prime}49^{\prime\prime}$ &~~~~~~ 19.9 & ~~~~2 &5210; z
= 3.3?  \cr 
\+1944.4$-$1436 && D   & 19 ~44 ~27.4 & ~~~$-$14 36 43 &~~~~~~ 19.3 &~~~~5
& \cr 
\+1944.6$-$1435 && E   & 19 ~44 ~39.8 & ~~~$-$14 35 17 &~~~~~~ 20.1 &~~~~4
& \cr 
\+1944.8$-$1511 && R   & 19 ~44 ~48.9 & ~~~$-$15 11 35 &~~~~~~ 19.7 &~~~~4
&5100,4020 \cr 
\+1945.0$-$1441 && L   & 19 ~45 ~01.0 & ~~~$-$14 41 35 &~~~~~~ 19.9 &~~~~3
&5225 \cr 
\+1945.0$-$1439 && J   & 19 ~45 ~02.8 & ~~~$-$14 39 13 &~~~~~~ 18.9 &~~~~4
&white dwarf? \cr 
\+1945.0$-$1457 && U   & 19 ~45 ~04.7 & ~~~$-$14 57 31 &~~~~~~ 19.0 &~~~~6
&H II? \cr 
\+1945.1$-$1436 && G   & 19 ~45 ~06.0 & ~~~$-$14 36 40 &~~~~~~ 18.1 &~~~~3
& \cr 
\+1945.0$-$1452 && E98 & 19 ~45 ~00.3 & ~~~$-$14 52 11 &~~~~~~ 20.3 &~~~~4
& \cr 
\+1945.4$-$1448 && B   & 19 ~45 ~26.6 & ~~~$-$14 48 58 &~~~~~~ 18.3 &~~~~4
& \cr 
\+1945.7$-$1429 && A   & 19 ~45 ~47.1 & ~~~$-$14 29 40 &~~~~~~ 18.4 &~~~~4
&white dwarf?  \cr 
\+1945.8$-$1437 && I   & 19 ~45 ~53.0 & ~~~$-$14 37 18 &~~~~~~ 17.6 &~~~~4
& \cr 
\vskip 3pt
\hrule
\vskip 8pt
\noindent
$^a$ estimated wavelengths given in order of decreasing intensity

\noindent
$^b$ tabulated redshifts estimated from grens spectra; 
~* indicates note at end of table
\vskip 5pt
\noindent
\ub{Notes:}
\vskip 5pt
\leftline{NGC 253 - H: identical to MS 00433-2531; z = 0.861 (Garilli et
al.\ 1992)} 
\leftline{NGC 253 - S: z = 2.521 (Clowes \& Savage 1983)}
\leftline{IC 1613 - P: z = 1.909 (Chaffee et al.\ 1991)}
\leftline{IC 1613 -B: very faint; 2 lines, but wavelength scale uncertain}
\leftline{NGC 2366 - P: z = 0.111; [O II], H$\beta$, [O III], H$\alpha$ }
\leftline{NGC 2403 - S: z = 1.76; Ly$\alpha$, [Si IV], C IV}
\leftline{NGC 2403 - O: z = 2.53; Ly$\alpha$, Ly$\beta$, C IV}
\leftline{NGC 2403 - R: z = 1.924; Ly$\alpha$, [N V], [Si IV], C IV, C
III]; identical to 0730+65W1;} 
\leftline{~~~~~~~~~~~~~~~~~~~~~~~~~~z = 1.927 (Tytler \& Fan 1992)}
\leftline{NGC 2403 - D: z = 2.24; Ly$\alpha$, [Si IV], C IV }
\leftline{NGC 2403 - N: z = 2.58; Ly$\alpha$, [Si IV], C IV }
\leftline{NGC 2403 - Q: quasar with one unidentified line at 4190\AA}
\leftline{NGC 2403 - U: z = 2.81; Ly$\alpha$, Ly$\beta$, [N V]}

\bye


